Mercury and OrbFit packages for the numerical integration of planetary systems: implementation of the Yarkovsky and YORP effects

For studies of the long-term evolution of small Solar System objects, it is fundamental to add the Yarkovsky and Yarkovsky-O'Keefe-Radzievskii-Paddack (YORP) effects in the dynamical model. Still, implementations of these effects in publicly available N-body codes are often lacking, or the effects are implemented using significantly simplified models. In this paper, we present an implementation of the coupled Yarkovsky/YORP effects in the mercury and OrbFit $N$-body codes. Along with these two effects, we also included the effects of non-destructive collisions and rotationally induced breakups to model the asteroid spin state properly. Given the stochastic nature of many incorporated effects, the software is suitable for statistical dynamical studies. Here we explained the scientific aspect of the implementation, while technical details will be made freely available along with the source codes.

==> abr_saj.tex <==
\newcommand\aap{A\&A}%     % Astronomy and Astrophysics 
\newcommand\aapr{A\&ARv}%  % Astronomy and Astrophysics Reviews 
\newcommand\aaps{A\&AS}%    % Astronomy and Astrophysics, Supplement 
\newcommand\aas{AAS Meeting Abstracts}% American Astronomical Society Meeting 
%Abstracts
\newcommand\actaa{AcA}%  % Acta Astronomica
\newcommand\aj{AJ}%        % Astronomical Journal 
\newcommand\ao{ApOpt}%   % Applied Optics ++
\newcommand\apj{ApJ}%    % Astrophysical Journal ++
\newcommand\apjl{ApJL}     % Astrophysical Journal, Letters 
\newcommand\apjs{ApJS}%    % Astrophysical Journal, Supplement 
\newcommand\aplett{Astrophys.~Lett.}%  % Astrophysics Letters 
\newcommand\apspr{Astrophys.~Space~Phys.~Res.}% % Astrophysics Space Physics 
%Research 
\newcommand\apss{Ap\&SS}%  % Astrophysics and Space Science 
\newcommand\araa{ARA\&A}%  % Annual Review of Astron and Astrophys 
\newcommand\azh{AZh}%       % Astronomicheskii Zhurnal 
\newcommand\baas{BAAS}%     % Bulletin of the AAS 
\newcommand\bac{Bull. astr. Inst. Czechosl.}
\newcommand\bain{BAN}% % Bulletin Astronomical Institute of the Netherlands 
\newcommand\caa{ChA\&A}%  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{ChJA\&A}%  % Chinese Journal of Astronomy and Astrophysics
\newcommand\dps{AAS/DPS Meeting Abstracts}% American Astronomical 
%Society/Division for Planetary Sciences Meeting Abstracts
\newcommand\fcp{FCPh}%   % Fundamental Cosmic Physics 
\newcommand\gca{GeoCoA}% % Geochimica Cosmochimica Acta 
\newcommand\grl{Geophys.~Res.~Lett.}%  % Geophysics Research Letters 
\newcommand\iaucirc{IAUC}% % IAU Cirulars 
\newcommand\icarus{Icar}% % Icarus
\newcommand\jcap{JCAP}%  % Journal of Cosmology and Astroparticle Physics
\newcommand\jcp{JChPh}%     % Journal of Chemical Physics 
\newcommand\jgr{JGR}%     % Journal of Geophysics Research 
\newcommand\jqsrt{JQSRT}%   % Journal of Quantitiative Spectroscopy and 
%Radiative Trasfer 
\newcommand\jrasc{JRASC}%   % Journal of the RAS of Canada 
\newcommand\maps{M\&PS}% Meteoritics and Planetary Science
\newcommand\memras{MmRAS}%  % Memoirs of the RAS 
\newcommand\memsai{MmSAI}% % Mem. Societa Astronomica Italiana 
\newcommand\mnras{MNRAS}%   % Monthly Notices of the RAS 
\newcommand\na{NewA}%  % New Astronomy
\newcommand\nar{NewAR}%  % New Astronomy Review
\newcommand\nat{Natur}%  % Nature 
\newcommand\nphysa{NuPhA}%     % Nuclear Physics A 
\newcommand\pasa{PASA}%  % Publications of the Astron. Soc. of Australia
\newcommand\pasj{PASJ}%     % Publications of the ASJ 
\newcommand\pasp{PASP}%     % Publications of the ASP 
\newcommand\physrep{PhR}%       % Physics Reports 
\newcommand\physscr{PhyS}%        % Physica Scripta 
\newcommand\planss{Planet.~Space~Sci.}%  % Planetary Space Science 
\newcommand\pra{PhRvA}% % Physical Review A: General Physics ++
\newcommand\prb{PhRvB}% % Physical Review B: Solid State ++
\newcommand\prc{PhRvC}% % Physical Review C ++
\newcommand\prd{PhRvD}% % Physical Review D ++
\newcommand\pre{PhRvE}% % Physical Review E ++
\newcommand\prl{PhRvL}% % Physical Review Letters 
\newcommand\procspie{Proc.~SPIE}%      % Proceedings of the SPIE 
\newcommand\qjras{QJRAS}%   % Quarterly Journal of the RAS 
\newcommand\rmxaa{RMxAA}%  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{S\&T}%   % Sky and Telescope 
\newcommand\solphys{SoPh}% % Solar Physics 
\newcommand\sovast{Soviet~Ast.}% % Soviet Astronomy 
\newcommand\ssr{SSRv}% % Space Science Reviews 
\newcommand\zap{ZA}%       % Zeitschrift fuer Astrophysik 

\let\astap=\aap 
\let\apjlett=\apjl 
\let\apjsupp=\apjs 
\let\applopt=\ao 





==> astro.tex <==
\def\tg{\mathop{\rm tg}\nolimits}
\def\arctg{\mathop{\rm arctg}\nolimits}

\def\point#1{\hbox{\setbox7=\hbox to0.6em{\hfil.\hfil}%
\setbox8=\hbox to0.5em{\hfil$^{#1}$\hfil}%
\box7\kern-0.5em\box8}}

\def\dan{\point{\rm d}}
\def\cas{\point{\rm h}}
\def\minut{\point{\rm m}}
\def\sekund{\point{\mathrm{s}}}

\def\oo{\point{\circ}}
\def\ll{\point{\prime}}
\def\uu{\point{\prime\prime}}




==> mjyu.tex <==
\def\nava{\leavevmode\hbox{,\kern-0.09em,}}%yu-navodnik-pocetni
\def\navb{\char'134}                                      %yu-navodnik-krajnji
\def\DJ{\leavevmode\setbox0=\hbox{D}\kern0pt
 \rlap{\kern.04em\raise.188\ht0\hbox{-}}D}
\def\dj{\leavevmode\setbox0=\hbox{d}\kern0pt
 \rlap{\kern.215em\raise.46\ht0\hbox{-}}d}
\def\SH{\v S} \def\sh{\v s} % Sasinci
\def\CJ{\' C} \def\cj{\' c} % Cicevac
\def\CH{\v C} \def\ch{\v c} % Xaxak
\def\Z{\v Z} \def\z{\v z} % Zuzemberk
\def\br{\break}



==> wncyr.tex <==
\def\rrmd{\font\tipo=wncyr12\tip}%
\def\rbfd{\font\tipo=wncyb12\tip}%
\def\rssd{\font\tipo=wncyss12\tip}%
\def\rrm{\font\tipo=wncyr10\tip}%
\def\rbf{\font\tipo=wncyb10\tip}%
\def\rit{\font\tipo=wncyi10\tip}%
\def\rss{\font\tipo=wncyss10\tip}%
\def\rsc{\font\tipo=wncysc10\tip}%
\def\rrmdev{\font\tipo=wncyr9\tip}%
\def\rbfdev{\font\tipo=wncyb9\tip}%
\def\ritdev{\font\tipo=wncyi9\tip}%
\def\rssdev{\font\tipo=wncyss9\tip}%
\def\rrmos{\font\tipo=wncyr8\tip}%
\def\rbfos{\font\tipo=wncyb8\tip}%
\def\ritos{\font\tipo=wncyi8\tip}%
\def\rssos{\font\tipo=wncyss8\tip}%
\def\rrmsev{\font\tipo=wncyr7\tip}%
\def\rbfsev{\font\tipo=wncyb7\tip}%
\def\ritsev{\font\tipo=wncyi7\tip}%
\def\tip{\relax\tipo\def\DD{\tipo\char'006}\def\dd{\tipo\char'016}% \tip
\def\DJ{\DD}\def\dj{\dd}% 
\def\ZZ{\tipo\char'021}\def\zz{\tipo\char'031}%
\def\Z{\ZZ}\def\z{\zz}%
\def\LJ{\tipo\char'001}\def\lj{\tipo\char'011}%
\def\NJ{\tipo\char'000}\def\nj{\tipo\char'010}%
\def\CC{\tipo\char'007}\def\cc{\tipo\char'017}%
\def\DZ{\tipo\char'002}\def\dz{\tipo\char'012}%
\def\XX{Q}\def\xx{q}%
\def\JJ{J}\def\jj{j}% 
\def\SS{X}\def\ss{x}%
\def\JA{\tipo\char'027}\def\ja{\tipo\char'037}%
\def\SC{W}\def\sc{w}%
\def\CJ{\CC}\def\cj{\cc}%
\def\CH{Q}\def\ch{q}%
\def\SH{X}\def\sh{x}%
% sch="x"; tvrdo i = "y"; ja = "j"; schtsch = "w"; tsch = "q"
\def\EE{\tipo\char'003}\def\ee{\tipo\char'013}% "e oborotnoe"
\def\JI{\tipo\char'022}\def\ji{\tipo\char'032}% rusko "j"
\def\JU{\tipo\char'020}\def\ju{\tipo\char'030}%
\def\M{\tipo\char'136}\def\m{\tipo\char'176}% meki znak
\def\TV{\tipo\char'137}\def\tv{\tipo\char'177}% tvrdi znak
\def\rnava{\tipo\char'074}\def\rnavb{\tipo\char'076}% ruski navodnici
\def\snava{\leavevmode\hbox{,\kern-0.06em,}}% yu-
\def\snavb{\tipo\char'134}}% navodnici
\def\br{\break}%



